OptEMA: Adaptive Exponential Moving Average for Stochastic Optimization with Zero-Noise Optimality

Exponential moving averages (EMAs) are a central component of widely used adaptive optimizers such as Adam. However, existing analyses of Adam-style methods often yield suboptimal guarantees in the zero-noise regime, rely on open-loop parameter schedules, or require prior knowledge of smoothness constants. Motivated by these limitations, we introduce OptEMA and analyze two complementary variants: OptEMA-M, which applies an adaptive, decreasing EMA coefficient to the first moment with a fixed second-moment decay, and OptEMA-V, which swaps these roles. At the heart of these variants is a Corrected AdaGrad-Norm coefficient schedule. This formulation renders OptEMA algorithmically closed-loop and Lipschitz-free, meaning its effective stepsizes are trajectory-dependent and require no parameterization via the Lipschitz constant. Under lower-boundedness, unbiasedness, bounded variance, average smoothness, and a bounded stochastic-gradient condition used to control the adaptive normalizers, we prove that both variants achieve the unified noise-adaptive rate $\tilde{\mathcal{O}} \left(T^{-1/2}+\sigma^{1/2}T^{-1/4}\right)$ for the averaged gradient norm. In the zero-noise regime, these bounds automatically reduce to the nearly optimal deterministic rate $\widetilde{\mathcal{O}}(T^{-1/2})$ without manual hyperparameter retuning.

==> myinit.tex <==
\usepackage{graphicx}
\usepackage{epstopdf}



\usepackage{enumitem,amsfonts,amssymb,mathtools,bm,pifont,bbm,listings,xcolor,threeparttable,xcolor}
\usepackage{ulem,hyperref,comment,amsmath}
%\let\proof\relax       % �������е� proof ����
%\let\endproof\relax    % �������е� endproof ����
%\usepackage{amsthm}    % ���¼��� amsthm
%\let\algorithm\relax
%\let\endalgorithm\relax
%\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
%\usepackage{algpseudocode}
%amsthm subcaption
%\usepackage{natbib}
\usepackage{natbib}
\usepackage{multirow}

% subcaption,algpseudocode,
% For Proofs
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{fact}[theorem]{Fact}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
%\newtheorem{remark}[theorem]{Remark}


%\allowdisplaybreaks
% Letters
% Commonly used notations
%\usepackage{verbatim}
\def\trans{^\mathsf{T}}\def\Rn{\mathbb{R}} \def\one{\mathbf{1}} \def\zero{\mathbf{0}}\def\sign{\mathrm{sign}}
\def\trans {^\mathsf{T}}
\def\fro {\mathsf{F}}



% \definecolor{mydarkgreen}{RGB}{5,81,23}
\definecolor{mydarkgreen}{RGB}{39,130,67}
\definecolor{mydarkred}{RGB}{192,25,25}
%\newcommand{\green}{\color{mydarkgreen}}
%\newcommand{\red}{\color{mydarkred}}
% \newcommand{\blue}{\color{mydarkblue}}
%\newcommand{\cmark}{\green\ding{51}}%
%\newcommand{\xmark}{\red\ding{55}}%

\usepackage{relsize} %SEB: feel free to revert, I think the font looked a bit too big otherwise
%\xspace

%\def\vec{\operatorname*{vec}}
\DeclareMathOperator{\st}{s.t.}
\DeclareMathOperator{\mat}{mat}
\DeclareMathOperator{\avg}{avg}
%\DeclareMathOperator{\vecc}{vec}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\crit}{Crit}
\DeclareMathOperator{\Prox}{\operatorname{Prox}}
\DeclareMathOperator{\argmin}{arg\,min}
\newcommand{\diam}{\mathrm{diam}}


\newcommand{\beq}{\begin{eqnarray}}
\newcommand{\eeq}{\end{eqnarray}}
\newcommand{\beqq}{\begin{equation}}
\newcommand{\eeqq}{\end{equation}}
%\newcommand{\bel}{\[\begin{aligned}}
%\newcommand{\eel}{\end{aligned}\]}
\newcommand{\bel}{\begin{align}}
\newcommand{\eel}{\end{align}}
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\noi}{\noindent}
\newcommand{\nn}{\nonumber}
\def\noi{\noindent}
\def\nn{\nonumber}
\def\la{\langle}
\def\ra{\rangle}
\def\diag{{\rm{diag}}}
\def\Diag{{\rm{Diag}}}
\def\dist{{\rm{dist}}}
\newcommand{\step}[1]{\text{\ding{\numexpr#1+171\relax}}}
%\newcommand{\tfractt}{\tfrac}

% Greek alphabet
\def\nablas{\boldsymbol{\nabla}}
\def\Deltas{\boldsymbol{\Delta}}
\def\etas{\boldsymbol{\eta}}
\def\epsilons{\boldsymbol{\epsilon}}
\def\varepsilons{\boldsymbol{\varepsilon}}
\def\xis{\boldsymbol{\xi}}
\def\zetas{\boldsymbol{\zeta}}
\def\lambdas{\boldsymbol{\lambda}}
\def\ts{\textstyle}

\def\cone{\textcolor[rgb]{0.9961,0,0}}
\def\ctwo{\textcolor[rgb]{0,0.7,0}}
\def\cthree{\textcolor[rgb]{0,0.5820,0.9}}


\def\cc{\mathbf{c}}\def\a{\mathbf{a}}\def\b{\mathbf{b}}\def\d{\mathbf{d}}\def\e{\mathbf{e}}\def\f{\mathbf{f}}\def\g{\mathbf{g}}\def\h{\mathbf{h}}\def\i{\mathbf{i}}\def\j{\mathbf{j}}\def\k{\mathbf{k}}\def\l{\mathbf{l}}\def\m{\mathbf{m}}\def\n{\mathbf{n}}\def\o{\mathbf{o}}\def\p{\mathbf{p}}\def\q{\mathbf{q}}\def\r{\mathbf{r}}\def\s{\mathbf{s}}\def\t{\mathbf{t}}\def\u{\mathbf{u}}\def\v{\mathbf{v}}\def\w{\mathbf{w}}\def\x{\mathbf{x}}\def\y{\mathbf{y}}\def\z{\mathbf{z}}\def\A{\mathbf{A}}\def\B{\mathbf{B}}\def\C{\mathbf{C}}\def\D{\mathbf{D}}\def\E{\mathbf{E}}\def\G{\mathbf{G}}\def\H{\mathbf{H}}\def\I{\mathbf{I}}\def\J{\mathbf{J}}\def\K{\mathbf{K}}\def\M{\mathbf{M}}\def\N{\mathbf{N}}\def\O{\mathbf{O}}\def\P{\mathbf{P}}\def\Q{\mathbf{Q}}\def\R{\mathbf{R}}\def\S{\mathbf{S}}\def\T{\mathbf{T}}\def\U{\mathbf{U}}\def\V{\mathbf{V}}\def\W{\mathbf{W}}\def\X{\mathbf{X}}\def\Y{\mathbf{Y}}\def\Z{\mathbf{Z}}\def\v{\mathbf{v}}\def\p{\mathbf{p}}

\def\AA{\mathcal{A}}\def\BB{\mathcal{B}}\def\CC{\mathcal{C}}\def\DD{\mathcal{D}}\def\EE{\mathcal{E}}\def\FF{\mathcal{F}}\def\GG{\mathcal{G}}\def\HH{\mathcal{H}}\def\II{\mathcal{I}}\def\JJ{\mathcal{J}}\def\KK{\mathcal{K}}\def\LL{\mathcal{L}}\def\MM{\mathcal{M}}\def\NN{\mathcal{N}}\def\OO{\mathcal{O}}\def\PP{\mathcal{P}}\def\QQ{\mathcal{Q}}\def\RR{\mathcal{R}}\def\SS{\mathcal{S}}\def\TT{\mathcal{T}}\def\UU{\mathcal{U}}\def\VV{\mathcal{V}}\def\WW{\mathcal{W}}\def\XX{\mathcal{X}}\def\YY{\mathcal{Y}}\def\ZZ{\mathcal{Z}}

\def\AAA{\mathbb{A}}\def\BBB{\mathbb{B}}\def\CCC{\mathbb{C}}\def\DDD{\mathbb{D}}\def\EEE{\mathbb{E}}\def\FFF{\mathbb{F}}\def\GGG{\mathbb{G}}\def\HHH{\mathbb{H}}\def\III{\mathbb{I}}\def\JJJ{\mathbb{J}}\def\KKK{\mathbb{K}}\def\LLL{\mathbb{L}}\def\MMM{\mathbb{M}}\def\NNN{\mathbb{N}}\def\OOO{\mathbb{O}}\def\PPP{\mathbb{P}}\def\QQQ{\mathbb{Q}}\def\RRR{\mathbb{R}}\def\SSS{\mathbb{S}}\def\TTT{\mathbb{T}}\def\UUU{\mathbb{U}}\def\VVV{\mathbb{V}}\def\WWW{\mathbb{W}}\def\XXX{\mathbb{X}}\def\YYY{\mathbb{Y}}\def\ZZZ{\mathbb{Z}}
























%\newcommand{\tinytiny}{\fontsize{4}{4}\selectfont}
%\usepackage{accents}
%\usepackage{tikz}
%\def\halfcheckmark{\tikz\draw[scale=0.32,fill=black](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle (0.75,0.2) -- (0.77,0.2)  -- (0.3,0.6) -- cycle;}

%\renewcommand{\cite}{\citep}
%\newcommand{\fracpartial}[2]{\frac{\partial #1}{\partial  #2}}
%\usepackage{comment}




\def\NO{\ding{56}}
\def\YES{\ding{52}}



